Inverse Problem of Nonlinear Schr\"odinger Equation as Learning of Convolutional Neural Network

In this work, we use an explainable convolutional neural network (NLS-Net) to solve an inverse problem of the nonlinear Schr\"odinger equation, which is widely used in fiber-optic communications. The landscape and minimizers of the non-convex loss function of the learning problem are studied empirically. It provides a guidance for choosing hyper-parameters of the method. The estimation error of the optimal solution is discussed in terms of expressive power of the NLS-Net and data. Besides, we compare the performance of several training algorithms that are popular in deep learning. It is shown that one can obtain a relatively accurate estimate of the considered parameters using the proposed method. The study provides a natural framework of solving inverse problems of nonlinear partial differential equations with deep learning.

==> Analysis.tex <==
\section{Stability of inverse problem}
In this section, we prove the stability of the inverse problem. 
\begin{theorem}\label{thm:stab}
Let $\Omega=[t_1,t_2]$ be a specific time interval. Suppose  $\Ai(t)$ is the data at the transmitter. $\Ao^j(t)$ is data at the receiver corresponding to parameter $(\beta_j,\gamma_j)$, for $j=1,2$.  Then there exists positive constants $K_i$, $i=1,\ldots,3$ such that
the following estimates hold:
\begin{align}
|\gamma_1-\gamma_2|&\leq K_1\|\Ai(t)\|_{L^2(\Omega)},
\label{est_gamma}\\
|\beta_1-\beta_2|&\leq K_2(\|\Ao^1(t)-\Ao^2(t)\|_{L^2(\Omega)})+K_3\|\Ai(t)\|_{L^2(\Omega)}.
\label{est_beta}
\end{align}
\end{theorem}
\begin{proof}
 For $j=1,2$, we define that $A_j(t,z)$ to be the solution to the following equations
\begin{align}
\begin{cases}
\label{eq:diri bc}
    \frac{\p A_j}{\p z} =-\frac{i\beta_j}{2}\frac{\p^{2} A_j}{\p t^{2}} +i\gamma_j |A_j|^{2} A_j, & t\in\Omega, z\in [0,Z],\\
    A_j(t,0) = \Ai(t), & t\in\Omega,\\
    A_j=0, & t\in\p\Omega,z\in[0,Z],
\end{cases}
\end{align}
As introduced in \ref{ss:CNN}, we apply operator splitting to solve \cref{eq:diri bc}. Let $[0,Z]=\bigcup\limits_{i=1}^{2r}D_i$, where $D_i=[i\xi,(i+1)\xi]$. To prove the stability, we apply a simple version of operator splitting. In particular, we simply consider one operator on each $D_i$. We only use nonlinear operator $\cN$ on $D_p$, where $p=2s+1,\quad 0\leq s\leq r-1$. Otherwise, we only apply linear operator $\cL$. We define $B_{j}(t,z)$ to be the approximate solution to $A_j(t,z)$ corresponding to parameters $(\beta_j,\gamma_j)$ after applying the splitting approach defined above. In particular, for $j=1,2$, $B_j$ satisfies the following equations.
\begin{eqnarray}
\begin{aligned}
    \frac{\p B_j}{\p z}=i\gamma_j|B_j|^2B_j,\quad& t\in \Omega,z\in D_{p},  \\
      \frac{\p B_j}{\p z}=-\frac{i\beta_j}{2}\frac{\p^2 B_j}{\p t^2}, \quad& t\in \Omega,z\in D_{p+1},\label{eq:splitting bc}
\end{aligned}
\end{eqnarray}
where $p=2s+1,\quad 0\leq s\leq r-1$.

We first consider $D_1$.
 For $j=1,2$, we have
\begin{align}
\begin{cases}
\label{eq:diri_gamma}
    \frac{\p B_j}{\p z} =i\gamma_j |B_j|^{2} B_j, & t\in\Omega, z\in D_1\\
    B_j(t,0) = \Ai(t), & t\in\Omega,\\
    B_j(t,z)=0,& t\in\p\Omega, z\in D_1.
\end{cases}
\end{align}

We have
\begin{align}
    B_j(t,z)&=A^0\exp(i\gamma_j|A^0|^2z), 
\end{align}
where $z\in D_1$.
Define $I_1:=\|B_1(t,\xi)-B_2(t,\xi)\|_{L^2(\Omega)}$.
Then we have 
\begin{eqnarray}
\begin{aligned}
   I_1^2&=\|A^0(\exp(i\gamma_1|A^0|^2\xi)-\exp(i\gamma_2|A^0|^2\xi))\|_{L^2(\Omega)}^2=\|A^0(\exp(i(\gamma_1-\gamma_2)|A^0|^2\xi)-1)\|_{L^2(\Omega)}^2\\
    &=\displaystyle 4\int_{\Omega}\left|A^0\sin\frac{|A^0|^2(\gamma_1-\gamma_2)\xi}{2}\right|^2dt=4|\gamma_1-\gamma_2|^2
    \int_{\Omega} \frac{|A^0\sin\frac{|A^0|^2(\gamma_1-\gamma_2)\xi}{2}|^2}{|\gamma_1-\gamma_2|^2}dt.
\end{aligned}
\end{eqnarray}
We further define $\Omega_1=\{t:0<|\Ai(t)|^2|\gamma_1-\gamma_2|\xi<2\}$.
Hence, there exists a positive constant $C_1$ such that
\begin{align}
    I_1^2\geq |\gamma_1-\gamma_2|^2\int_{\Omega_1} \frac{1}{9}|A^0|^6\xi^2 dt\geq C_1|\gamma_1-\gamma_2|
    ^2.
\end{align}
By using triangle inequality, we have
\begin{eqnarray}
\begin{aligned}
I_1= \|B_1(t,\xi)-B_2(t,\xi)\|_{L^2(\Omega)}\leq\|B_1(t,\xi)\|_{L^2(\Omega)}+\|B_2(t,\xi)\|_{L^2(\Omega)}=2\|\Ai(t)\|_{L^2(\Omega)},
\end{aligned}
\end{eqnarray}
which completes the proof of \cref{est_gamma}.
To prove \cref{est_beta}, we consider $D_{2r}$.
\begin{align}
\begin{cases}
\label{eq:diri_beta}
    \frac{\p B_j}{\p z} =-\frac{i\beta}{2}\frac{\p^{2} B_j}{\p t^{2}}, & t\in\Omega, z\in D_{2r}\\
    B_j(t,Z-\xi) = A_j(t,Z-\xi), & t\in\Omega,\\
    B_j=0,\quad &t\in\p\Omega, z\in D_{2r},
\end{cases}
\end{align}
 We denote the Fourier transform of a function f by $\hat{f}.$
Define $\tilde{\Omega}$ to be the corresponding frequency domain associated with $\Omega$ after applying Fourier transform. Let $\hat{B}_1(\omega,z)$ and $\hat{B}_2(\omega,z)$ be the Fourier Transforms of $B_1(t,z)$ and $B_2(t,z)$, where $\omega\in \tilde{\Omega}$. We define $\hat{Q}_j=A_j(t,Z-\xi)$. From \eqref{eq:diri_beta}, we have
\begin{align}
    \hat{B}_1(\omega,Z-\frac{\xi}{2}+z)&=\hat{Q}_1\exp{\frac{iz \omega^2\beta_1}{2}},\\
    \hat{B}_2(\omega,Z-\frac{\xi}{2}+z)&=\hat{Q}_2\exp{\frac{iz \omega^2\beta_2}{2}}.
\end{align}
Define $I_2:=\|B_1(t,Z)-B_2(t,Z)\|_{L^2(\Omega)}.$
By Parseval's theorem, we have 
\begin{align*}
    I_2&=\|\hat{B}_1(t,Z)-\hat{B}_2(t,Z)\|_{L^2(\tilde{\Omega})}=\|\hat{Q}_1\exp{\frac{i\xi \omega^2\beta_1}{2}}-\hat{Q}_2\exp{\frac{i\xi \omega^2\beta_2}{2}}\|_{L^2(\tilde{\Omega})}\\
   &\geq \|\hat{Q}_1(\exp{\frac{i\xi \omega^2(\beta_1-\beta_2)}{2}}-1)\|_{L^2(\tilde{\Omega})}-\|\hat{Q}_1-\hat{Q}_2\|_{L^2(\tilde{\Omega})}\\
   &=\|\hat{Q}_1(\exp{\frac{i\xi \omega^2(\beta_1-\beta_2)}{2}}-1)\|_{L^2(\tilde{\Omega})}-\|Q_1-Q_2\|_{L^2(\Omega)}
\end{align*}
Define $S:=\|\hat{Q}_1(\exp{\frac{i\xi \omega^2(\beta_1-\beta_2)}{2}}-1)\|_{L^2(\tilde{\Omega})}$ and we have
\begin{align}
    S^2=4\int_{\tilde{\Omega}}\left|\hat{Q}_1\sin \frac{\xi \omega^2(\beta_1-\beta_2)}{4}\right|^2d\omega
    =4|\beta_1-\beta_2|^2\int_{\tilde{\Omega}}\frac{|\hat{Q}_1\sin \frac{\xi \omega^2(\beta_1-\beta_2)}{4}|^2}{|\beta_1-\beta_2|^2}d\omega
\end{align}
Define $\Omega_2=\{\omega:0<\xi \omega^2|\beta_1-\beta_2|<4\}$.
Hence, there exists a positive constant $C_2$ such that
\begin{align}
    S^2\geq |\beta_1-\beta_2|^2\int_{\tilde{\Omega}}|\frac{5}{24}\xi\omega^2\hat{Q}_1|^2d\omega\geq C_2|\beta_1-\beta_2|^2.
\end{align}
Using triangle inequality, we have
\begin{eqnarray}
\begin{aligned}
\|Q_1-Q_2\|_{L^2(\Omega)}\leq 2\|\Ai\|_{L^2(\Omega)}.
\end{aligned}
\end{eqnarray}
Hence there exists positive constants $K_2$ and $K_3$
\begin{eqnarray}
\begin{aligned}
|\beta_1-\beta_2|\leq K_2\|\Ao^1(t)-\Ao^2(t)\|_{L^2(\Omega)}+K_3\|\Ai(t)\|_{L^2(\Omega)},
\end{aligned}
\end{eqnarray}
where we use $B_j(t,Z)$ to be approximation to $\Ao^j(t)$.
\end{proof}

